Dynamic System Identification, and Control for a cost effective open-source VTOL MAV

This paper describes dynamic system identification, and full control of a cost-effective vertical take-off and landing (VTOL) multi-rotor micro-aerial vehicle (MAV) --- DJI Matrice 100. The dynamics of the vehicle and autopilot controllers are identified using only a built-in IMU and utilized to design a subsequent model predictive controller (MPC). Experimental results for the control performance are evaluated using a motion capture system while performing hover, step responses, and trajectory following tasks in the present of external wind disturbances. We achieve root-mean-square (RMS) errors between the reference and actual trajectory of x=0.021m, y=0.016m, z=0.029m, roll=0.392deg, pitch=0.618deg, and yaw=1.087deg while performing hover. This paper also conveys the insights we have gained about the platform and returned to the community through open-source code, and documentation.

==> contribs/Discussion.tex <==
% !TEX root = ../ICRA2017_DJI_sysid.tex
\section{Discussion and Limitations}
The works presented in this paper only address a point-level segmentation and have not been integrated into the real sweet pepper picking system. We thus do not have measures of the effectiveness/usefulness of the proposed method. This will be assessed shortly after incorporating the proposed system with ROS (e.g., successful picking rate with/without the method). 

Another noticeable limitation of the proposed system is that the trained model yields false positives for other stems and leaves that exhibit similar colour and shape to the peduncle as shown in Fig.~\ref{fig:detection_quatitative_results_with_background}. To overcome this issue, we will make use of context features that take into account the relationship between a sweet pepper and a peduncle. We will calculate a vector between the centroid of a sweet pepper and a point segmented as a peduncle with respect to the gravity vector. With this extra information the supervised learning algorithm will likely be able to determine that peduncles are usually above the centroid at a within a range of distances, improving the false positive rate. The accompanying video demonstration displays the qualitative results in different viewing points\footnoteref{foot:video_data}.
